Intention is All You Need: Refining Your Code from Your Intention

Code refinement aims to enhance existing code by addressing issues, refactoring, and optimizing to improve quality and meet specific requirements. As software projects scale in size and complexity, the traditional iterative exchange between reviewers and developers becomes increasingly burdensome. While recent deep learning techniques have been explored to accelerate this process, their performance remains limited, primarily due to challenges in accurately understanding reviewers' intents. This paper proposes an intention-based code refinement technique that enhances the conventional comment-to-code process by explicitly extracting reviewer intentions from the comments. Our approach consists of two key phases: Intention Extraction and Intention Guided Revision Generation. Intention Extraction categorizes comments using predefined templates, while Intention Guided Revision Generation employs large language models (LLMs) to generate revised code based on these defined intentions. Three categories with eight subcategories are designed for comment transformation, which is followed by a hybrid approach that combines rule-based and LLM-based classifiers for accurate classification. Extensive experiments with five LLMs (GPT4o, GPT3.5, DeepSeekV2, DeepSeek7B, CodeQwen7B) under different prompting settings demonstrate that our approach achieves 79% accuracy in intention extraction and up to 66% in code refinement generation. Our results highlight the potential of our approach in enhancing data quality and improving the efficiency of code refinement.

==> src/draft.tex <==
\section{Introduction}

% Code review是什么。很重要。 耗费很多人力，需要自动化。

% code refine是什么。 已有一些工作证明了，LLM技术在coderefine任务中的效果不错。然而总体效果仍不理想。

% 有两方面原因，第一是输入数据不全，第二是prompt设计过于简单。

% 输入方面：传统的输入只是old code和review comment。但这是一个复杂的流程，developer是可以感知到当前项目的所有信息的，其中两个至关重要的信息是last diff和review line。对于一个review质疑上次commit的必要性，是需要revert到上次修改前的状态。而有些review只是简单的说删除这一行，这是需要review所指的具体哪一行的信息的。

% prompt方面：随着LLM prompt技术的发展，有更多的prompt技术在NLP领域和软工领域都有很好的效果。如问答，数学求解，代码生成，测试用例生成等。包括了single agent的 cot， fewshot， self-gen等，还包括了multi-agent的xxx，yyy等。这些技术会对code refine有什么效果，这些也是关键问题。

% 基于以上原因，我们先做了一个empirical study。尝试了在多输入信息的情况下，用现有个prompt技术的效果。得到以下结论
% 1. 对于不同的任务类型，需要的信息不同
% 2. 对于不同的任务类型，需要的prompt策略也不同

% 基于以上发现，我们设计了一种新的multi-agent的检测框架。首先将任务分类，然后对不同类型可以设计不同的输入，以及不同promnpt策略。最后，使用多轮检测的MA技术，提高了整体EM值。

% 我们的主要贡献有：
% 1. 重新定了一种coderefine任务。增加了新的输入信息，更加贴近真实场景，更加实用
% 2. 调研了现有prompt技术在
% 3. 提出一种framework，提高了coderefine效果

\section{Background}

\subsection{Code refine}
% 形式化定义, input: original code, last diff, review line, review comment
% output: new code


\subsection{Prompt Engineering}
% prompt 技巧包括：COT， one-shot, fewshot
% Single angent 和 Multi agent
% In 0-shot prompting, φ directly yields x
% In 0-shot CoT, φ supplements x with a general instruction, such as “[x] think step by step”.
% In few-shot CoT, φ supplements x with several labeled exemplars, {(xi,ri,ai)}K
% i=1, such as “[x1] [r1] [a1]...[xK ] [rK ] [aK ] [x]”.

\section{Empirical Exploration}
% 经验研究的目标是，分析现有prompt engineer方法在全量code refine任务上的效果。

% The empirical study aims to investigate LLM 在 code review 任务中的效果，有哪些优点和不足。为了达成这个目标，我们设计了以下RQ
% 数据收集流程：
% 1. 可以获得的信息：original code, last diff, review line, review comment等。现有数据集的情况。
% 2. 数据质量问题，即自动化处理的边界（观察review和commit之间，一对多，多对一的情况）
% 3. 数据分类：

% RQ1 现有prompt工程方法的效果
% 1 单轮prompt的技巧：COT, fewshot, retrival-fewshot，self-gen
% 2 multi-agent方法：6*6

% 结论：
% 1. 不同类型的任务，需要的信息不同，需要不同的prompt方法
% 3. 检测者能力很弱，难以利用多轮对话提高效果


\section{Method}

\section{Experimental Setup}

% RQ2 框架的效果
% 1 按类别设计的prompt的效果
% 2 按类别设计checker的效果
% 3 分类的效果
% 4 总体效果/每一轮的效果


\section{Experimental result}

\subsection{dataset}
\subsection{result}

\section{related work}

% 有研究表明，generating review comment任务往往只能生成一些简单的review comment，如replace operator，remove exception, rename等，平均comment长度在6个words左右。而对于一些复杂的任务，如refactoring，performance optimizations等，特别是那些长度多于14个单词的review comment，生成效果很差。

% 为了使得codereview自动化，许多工作主要围绕以下两个任务，生成评论和代码修改。生成评论是xxxx，代码修改是xxxxx。
% 最早，由Tufano实现了一个基于NMT的自动化，处理java code review的问题。后来Tu还做了xxxx等工作
% 后来，微软实现了预训练模型，可以深刻理解代码片段
% 总体而言，他们对于代码修改任务的输入还只是comment+oldcode。一方面这受限于当时的模型输入长度，另一方面

% codereview包括生成评论和代码修复两部分工作。comment生成任务是很难自动化的，一方面这是由于现有模型的能力不足。现有模型只有能力完成一些添加/移出异常，更改变量名等简单任务。对于真正设计核心的逻辑的修改毫无办法，最后一些已经上线到github的自动化comment生成的工具，被developer采纳的概率也不高。另一方面，这个问题应该前移到代码生成，或者代码检查任务中。完整的代码结构，项目信息可以加强模型对当前代码的理解能力，可以生成更好的comment。另外，developer可以立即得到comment，可以即时修改反馈。
% 我们的研究重点在于代码修复部分。代码修复是指xxxx。而代码修复的自动化包括了LLM和pretrained-model两种。
% 一些研究表明，相比pretainedmodel, LLM在代码修复中有很好的效果。主要有两个原因，第一是数据质量比较低，依次作为训练集会影响效果。第二是code refine任务需要理解当前代码内容以及review的意图，这中复杂的理解能力是LLM更擅长的。
